Future constraints on halo thermodynamics from combined Sunyaev-Zel'dovich measurements

The improving sensitivity of measurements of the kinetic Sunyaev-Zel'dovich (SZ) effect opens a new window into the thermodynamic properties of the baryons in halos. We propose a methodology to constrain these thermodynamic properties by combining the kinetic SZ, which is an unbiased probe of the free electron density, and the thermal SZ, which probes their thermal pressure. We forecast that our method constrains the average thermodynamic processes that govern the energetics of galaxy evolution like energetic feedback across all redshift ranges where viable halos sample are available. Current Stage-3 cosmic microwave background (CMB) experiments like AdvACT and SPT-3G can measure the kSZ and tSZ to greater than 100$\sigma$ if combined with a DESI-like spectroscopic survey. Such measurements translate into percent-level constraints on the baryonic density and pressure profiles and on the feedback and non-thermal pressure support parameters for a given ICM model. This in turn will provide critical thermodynamic tests for sub-grid models of feedback in cosmological simulations of galaxy formation. The high fidelity measurements promised by the next generation CMB experiment, CMB-S4, allow one to further sub-divide these constraints beyond redshift into other classifications, like stellar mass or galaxy type.

==> makefile <==
# Makefile to produce the article.
LATEX  =  TEXINPUTS=.//: BSTINPUTS=.//: latex
PDFLATEX  = pdflatex -shell-escape 
DVIPS  =  dvips
PSPDF  =  ps2pdf
FIGURES = figures/

.PRECIOUS: $(FIGURES)

default: kSZ_energetics.pdf

%.pdf : $(FIGURES) %.tex
	$(PDFLATEX) $*.tex	
	TEXINPUTS=:.// BSTINPUTS=:.// bibtex $*
	$(PDFLATEX) $*.tex
	$(PDFLATEX) $*.tex
	$(PDFLATEX) $*.tex
#	$(DVIPS) -o $*.ps $*.dvi
#	$(PSPDF) $*.ps $*.pdf
	make clean

clean:
	rm -f *.log *.toc *.aux *.bak *.blg *.obj *.out

realclean:
	rm -f *.log *.toc *.aux *.obj *.bak *.bbl *.blg *.brf \
              *~ */*~ *.bak */*.bak 

